A Bayesian spatio-temporal model of panel design data: airborne particle number concentration in Brisbane, Australia

This paper outlines a methodology for semi-parametric spatio-temporal modelling of data which is dense in time but sparse in space, obtained from a split panel design, the most feasible approach to covering space and time with limited equipment. The data are hourly averaged particle number concentration (PNC) and were collected, as part of the Ultrafine Particles from Transport Emissions and Child Health (UPTECH) project. Two weeks of continuous measurements were taken at each of a number of government primary schools in the Brisbane Metropolitan Area. The monitoring equipment was taken to each school sequentially. The school data are augmented by data from long term monitoring stations at three locations in Brisbane, Australia. Fitting the model helps describe the spatial and temporal variability at a subset of the UPTECH schools and the long-term monitoring sites. The temporal variation is modelled hierarchically with penalised random walk terms, one common to all sites and a term accounting for the remaining temporal trend at each site. Parameter estimates and their uncertainty are computed in a computationally efficient approximate Bayesian inference environment, R-INLA. The temporal part of the model explains daily and weekly cycles in PNC at the schools, which can be used to estimate the exposure of school children to ultrafine particles (UFPs) emitted by vehicles. At each school and long-term monitoring site, peaks in PNC can be attributed to the morning and afternoon rush hour traffic and new particle formation events. The spatial component of the model describes the school to school variation in mean PNC at each school and within each school ground. It is shown how the spatial model can be expanded to identify spatial patterns at the city scale with the inclusion of more spatial locations.

==> gmrfs.tex <==
\subsubsection{GMRF on a torus}
\textbf{This should be amended or deleted}.

To calculate the daily and weekly trend together, we define the GMRF of the temporal effects to have a graph which corresponds to a Toeplitz Block Circulant (TBC) matrix such that the neighbours of each node are the previous hourly measurement, the subsequent hourly measurement, the previous day's measurement at the same time and the subsequent day's measurement at the same time.

This enforces cyclic behaviour within each day and within each week, essentially mapping the 168 hours of the week to a torus (rather than to a rectangle if we didn't enforce periodicity at the boundaries of each and week).

The TBC matrix thus has $\mat{R}_{i,i} = 4$ (four neighbours per node), off-diagonals of $-1$ according to the pattern in \figref{fig:toeplitz} and is a $168 \times 168$ real valued matrix with rank deficiency of 1.
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{tbc.pdf}
\caption{Structure of a Toeplitz Block Circulant matrix for daily and weekly trends within a week. The off-diagonal elements are a distance of 1 and 24 elements from the diagonal.}
\label{fig:toeplitz}
\end{figure}

\subsubsection{GMRF on a cylinder}
We are also interested in interaction effects where only one term requires cyclic behaviour, thus the resulting topology resembles a cylinder (as opposed to a torus). For example, in the interaction between wind speed and wind direction, the wind direction basis should be cyclic but the wind speed basis should not. 

For the cylindrical precision matrix, each block corresponding to a slice of the cylinder (one instance of the cyclic basis) will be TBC. The cylindrical matrix is constructed by making a block diagonal matrix of TBC blocks, adding the bands corresponding to the inter-block coprecisions (e.g. between two observations at the same wind heading one wind speed unit apart) and then ensuring that the diagonal elements are the number of neighbours; three in the case of the elements in slices on the top and bottom of the cylinder, four elsewhere. The precision matrix is banded (but not TBC because only one basis is cyclic) and has a rank deficiency of 1.

An example of a cylindrical precision matrix is given in \figref{fig:cylinder}.  R code to construct the cylindrical precision matrix is provided in the appendix.
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{cylinder.pdf}
\caption{Structure of the precision matrix for a regular 2D grid on a cylinder dividided into 11 slices and 8 polar directions. The uniform maximum bandwidth corresponds to the coprecision between two observations at the same wind heading one wind speed unit apart.}
\label{fig:cylinder}
\end{figure}


==> penalties.tex <==
The recursive construction of the $k^{\textnormal{th}}$ B-spline basis in $x$ is
\begin{equation}
\frac{B_{j,k}(x)}{t_{j+k}-t_{j}} = \frac{x - t_j}{t_{j+k-1}-t_{j}} \frac{B_{j,k-1}(x)}{t_{j+k-1}-t_{j}} +  \frac{t_{j+k} - x}{t_{j+k}-t_{j}} \frac{B_{j+1,k-1}(x)}{t_{j+k}-t_{j+1}} \label{eq:bs}
\end{equation}
with knots $t_i$, and initial condition $B_{j,0}(x) = 1$ \citep{deboor78}. The vectors produced by evaluating these basis functions at the covariate locations form the basis of the linear predictor matrix $\mat{X}$ with coefficients $\vec{\theta}$.

The penalty matrix for minimising the first derivative of three B-spline coefficients is constructed by taking the first derivative of the identity matrix
\[
\mat{D}^{(1)}_3 = \begin{bmatrix} -1 & 1 & 0 \\ 0  & -1 & 1 \end{bmatrix}
\]
and forming the product
\begin{equation}
\mat{K}^{(1)}_3 = \left( \mat{D}^{(1)}_3 \right)^T \mat{D}^{(1)}_3 = \begin{bmatrix} 1 & -1 & 0 \\ -1 & 2 & -1 \\ 0 & -1 & 1 \end{bmatrix} \label{eq:rw1}
\end{equation}
so that the quantity $\vec{\theta}^T \mat{K} \vec{\theta}$ is equal to the sum of the squares of the differential operator evaluated at $\vec{\theta}$ , e.g.
\begin{equation*}
\vec{\theta}^T \mat{K}_3^{(1)} \vec{\theta} = \left( \vec{\theta}^T  \left(\mat{D}^{(1)}_3\right)^T \right) \left( \mat{D}^{(1)}_3 \vec{\theta} \right)
 = \left\|  \mat{D}^{(1)}_3 \vec{\theta} \right\|^2  =  \sum_i \left( \mat{D}^{(1)}_3 \vec{\theta} \vert_{\theta_i} \right)^2
\end{equation*}
and taking the continuous limit results in the relationship
\begin{equation*}
\vec{\theta}^T \mat{K}_3^{(1)} \vec{\theta} \equiv \, \int \left( f^{(1)} (x) \right)^2 \, \textnormal{d}x
\end{equation*}
which holds for higher order penalties and is consistent with the frequentist interpretation of the spline penalty matrix \citep{wood00}. This can be thought of as a random walk penalty on the coefficients of the B-spline basis \citep{inla-jrssb09}.

